A hybrid machine learning framework for clad characteristics prediction in metal additive manufacturing

During the past decade, metal additive manufacturing (MAM) has experienced significant developments and gained much attention due to its ability to fabricate complex parts, manufacture products with functionally graded materials, minimize waste, and enable low-cost customization. Despite these advantages, predicting the impact of processing parameters on the characteristics of an MAM printed clad is challenging due to the complex nature of MAM processes. Machine learning (ML) techniques can help connect the physics underlying the process and processing parameters to the clad characteristics. In this study, we introduce a hybrid approach which involves utilizing the data provided by a calibrated multi-physics computational fluid dynamic (CFD) model and experimental research for preparing the essential big dataset, and then uses a comprehensive framework consisting of various ML models to predict and understand clad characteristics. We first compile an extensive dataset by fusing experimental data into the data generated using the developed CFD model for this study. This dataset comprises critical clad characteristics, including geometrical features such as width, height, and depth, labels identifying clad quality, and processing parameters. Second, we use two sets of processing parameters for training the ML models: machine setting parameters and physics-aware parameters, along with versatile ML models and reliable evaluation metrics to create a comprehensive and scalable learning framework for predicting clad geometry and quality. This framework can serve as a basis for clad characteristics control and process optimization. The framework resolves many challenges of conventional modeling methods in MAM by solving t the issue of data scarcity using a hybrid approach and introducing an efficient, accurate, and scalable platform for clad characteristics prediction and optimization.

==> tables/table-5-clf.tex <==
\begin{table}
\centering
\caption{Classification: cross validation accuracy and AUC values of the benchmark ML models for predicting the class of a clad.}
\label{tab:classification}
\begin{tabular}{ccc}
\toprule
Classifier Model  &  Accuracy\%  &  AUC  \\
\midrule
NN   &  92.90   &   94.59  \\
KNN   &  92.28   &   93.78  \\
GPC   &  90.74   &   92.81  \\
LR    &  91.97   &   94.48  \\
GNB   &  90.74   &   91.94 \\
SVC   &  88.29   &   90.60  \\
GBC   &  84.29   &   85.37  \\   
AB    &  80.58   &   80.07 \\ 
RF   &   89.50  &    88.57 \\
DT   &   88.89  &    69.12 \\ 
\bottomrule
\end{tabular}
\end{table}

==> tables/table-6-regression.tex <==
%\usepackage{booktabs}
\begin{table}
\centering
\caption{Regression: summary of $R^2$ and $MAE$ results of the benchmark ML models for clad width, height, and depth prediction.}
\label{tab:regression}
 \begin{tabular}{ccccccc}
\toprule
Regression
&
\multicolumn{2}{c}{Width}
&
\multicolumn{2}{c}{Height}
&
\multicolumn{2}{c}{Depth} \\\cmidrule(r){2-3}\cmidrule(l){4-5}\cmidrule(l){6-7}
Model & $R^2$ & $MAE$    & $R^2$ &$MAE$   & $R^2$   &$MAE$   \\
\bottomrule
NN   &   0.975  &   29.85  &   0.955  &   8.98   &   0.961  &   22.47  \\
GBR   &   0.985  &   24.41  &   0.964  &   8.73   &   0.981  &   19.96  \\
RF   &   0.981  &   33.28  &   0.952  &   11.41   &   0.972  &   23.43  \\
DT   &   0.975  &   42.00  &   0.875  &   18.53   &   0.927  &   32.61  \\
AB   &   0.958  &   48.23  &   0.849  &   20.53   &   0.945  &   32.75  \\
SVR   &   0.897  &  49.19  &   0.873  &   14.61   &   0.955  &   22.15  \\
GPR   &   0.915  &   56.72  &   0.879  &   18.37   &   0.957  &   24.87  \\
KNN    &   0.924  &   51.76  &   0.905  &   15.05   &   0.945  &   28.04  \\
Poly   &   0.969  &   40.64  &   0.912  &   17.11   &   0.964  &   23.41  \\
Lasso   &  0.825  &   95.35  &   0.731  &   23.88   &   0.886  &   49.62  \\
Ridge   &  0.825  &   95.34  &   0.731  &   23.88   &   0.886  &   49.63  \\
\bottomrule
\end{tabular}
\end{table}

